Thermal Activation of Methane by MgO$^+$: Temperature Dependent Kinetics, Reactive Molecular Dynamics Simulations and Statistical Modeling

The kinetics of MgO$^+$ + CH$_4$ was studied experimentally using the variable ion source, temperature adjustable selected ion flow tube (VISTA-SIFT) apparatus from 300 $-$ 600 K and computationally by running and analyzing reactive atomistic simulations. Rates and product branching fractions were determined as a function of temperature. The reaction proceeded with a rate of $k = 5.9 \pm 1.5 10^{-10}(T/300 $ K$)^{-0.5 \pm 0.2}$ cm$^3$ s$^{-1}$. MgOH$^+$ was the dominant product at all temperatures, but Mg$^+$, the co-product of oxygen-atom transfer to form methanol, was observed with a product branching fraction of $0.08 \pm 0.03 (T / 300 $ K$)^{-0.8 \pm 0.7}$. Reactive molecular dynamics simulations using a reactive force field, as well as a neural network yield rate coefficients about one order of magnitude lower. This underestimation of the rates is traced back to the multireference character of the transition state [MgOCH$_4$]$^+$. Statistical modeling of the temperature-dependent kinetics provides further insight into the reactive potential surface. The rate limiting step was found to be consistent with a four-centered activation of the C-H bond, consistent with previous calculations. The product branching was modeled as a competition between dissociation of an insertion intermediate directly after the rate-limiting transition state, and traversing a transition state corresponding to a methyl migration leading to a Mg-CH$_3$OH$^+$ complex, though only if this transition state is stabilized significantly relative to the dissociated MgOH$^+$ + CH$_3$ product channel. An alternative non-statistical mechanism is discussed, whereby a post-transition state bifurcation in the potential surface could allow the reaction to proceed directly from the four-centered TS to the Mg-CH$_3$OH$^+$ complex thereby allowing a more robust competition between the product channels.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}


